Parameter-Free Hypergraph Neural Network for Few-Shot Node Classification

Few-shot node classification on hypergraphs requires models that generalize from scarce labels while capturing high-order structures. Existing hypergraph neural networks (HNNs) effectively encode such structures but often suffer from overfitting and scalability issues due to complex, black-box architectures. In this work, we propose ZEN (Zero-Parameter Hypergraph Neural Network), a fully linear and parameter-free model that achieves both expressiveness and efficiency. Built upon a unified formulation of linearized HNNs, ZEN introduces a tractable closed-form solution for the weight matrix and a redundancy-aware propagation scheme to avoid iterative training and to eliminate redundant self information. On 11 real-world hypergraph benchmarks, ZEN consistently outperforms eight baseline models in classification accuracy while achieving up to 696x speedups over the fastest competitor. Moreover, the decision process of ZEN is fully interpretable, providing insights into the characteristic of a dataset. Our code and datasets are fully available at https://github.com/chaewoonbae/ZEN.

==> sections/035extension.tex <==
\subsection{Possible extensions for deeper propagation}
Some datasets may require models with higher-hop propagations for better expressivity. Without approximation, the exact computation of RSI requires high computational cost. One possible approximation is to estimate the probability that a random walker returns to the starting node after  steps, where  is the number of hops that we aim to model. 
A simple pseudocode for this strategy is provided in Algorithm~\ref{alg:self-info}.

% A simple pseudocode for this strategy is as follows:

% \begin{itemize}
%     \item Start at node $i$.
%     \item At each step:
%         \begin{enumerate}
%             \item Uniformly sample a hyperedge incident to the current node.
%             \item Uniformly sample a node connected to that hyperedge.
%         \end{enumerate}
%     \item Repeat this process for $l$ steps.
%     \item Record whether the walk ends at the original node $i$. The return probability may serve as an approximation of node-wise self-information at a given hop.
% \end{itemize}

\begin{algorithm}[t]
\caption{Approximation via random walks}
\label{alg:self-info}
\begin{algorithmic}[1]
\Require Node $i$, walk length $l$
\Ensure Return probability of node $i$
\State $count \gets 0$
\For{each trial}
    \State $current \gets i$
    \For{$t = 1$ \textbf{to} $l$}
        \State Sample a hyperedge $e$ incident to $current$ uniformly at random
        \State Sample a node $j$ connected to $e$ uniformly at random
        \State $current \gets j$
    \EndFor
    \If{$current = i$} 
        \State $count \gets count + 1$
    \EndIf
\EndFor
\State \Return $count / (\text{number of trials})$
\end{algorithmic}
\end{algorithm}


Another possible approximation is to use Hutchinson's Estimator, which provides an unbiased stochastic estimate of the diagonal entries. The equation is given by:
\begin{equation}
    \operatorname{diag}(\A) \approx \frac{1}{m}\sum_{k=1}^m \mathbf{z}^{(k)} \odot \left(\A \mathbf{z}^{(k)}\right)
\end{equation}
where $m$ is the number of random probe vectors, each $\mathbf{z}^{(k)} \in \mathbb{R}^n$ is a random vector with entries independently sampled from the Rademacher distribution (i.e., each entry is $+1$ or $-1$ with equal probability), and $\odot$ denotes the element-wise (Hadamard) product. The expectation satisfies $\operatorname{diag}(\A) = \mathbb{E}[\mathbf{z} \odot \left(\A \mathbf{z}\right)]$.

Hutchinson's Estimator does not require explicit storage of the entire matrix $\A$; instead, it relies solely on matrix-vector multiplications with randomized vectors $\mathbf{z}$. This characteristic renders Hutchinson's Estimator particularly suitable and computationally efficient for hypergraph structures. We consider these approaches to be promising directions for extending ZEN to scenarios where deeper propagation may provide additional benefits.
